Hostility Detection and Covid-19 Fake News Detection in Social Media

Withtheadventofsocialmedia,therehasbeenanextremely rapid increase in the content shared online. Consequently, the propagation of fake news and hostile messages on social media platforms has also skyrocketed. In this paper, we address the problem of detecting hostile and fake content in the Devanagari (Hindi) script as a multi-class, multi-label problem. Using NLP techniques, we build a model that makes use of an abusive language detector coupled with features extracted via Hindi BERT and Hindi FastText models and metadata. Our model achieves a 0.97 F1 score on coarse grain evaluation on Hostility detection task. Additionally, we built models to identify fake news related to Covid-19 in English tweets. We leverage entity information extracted from the tweets along with textual representations learned from word embeddings and achieve a 0.93 F1 score on the English fake news detection task.

==> table.tex <==



\begin{figure}[!h]
\begin{floatrow}
\RawFloats
\capbtabbox{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Class Name} & \textbf{Precision}        & \textbf{Recall} & \textbf{F1} & \textbf{Support} \\ \hline
Non-Hostile         & \cellcolor0.98 & 0.96            & 0.97        & 873              \\ \hline
Hostile             & 0.96                      & 0.97            & 0.97        & 780              \\ \hline
W.avg/Total         & 0.97                      & 0.97            & 0.97        & 1653             \\ \hline
\end{tabular}}{
\caption{Descriptions of mobile sensors present in both datasets.}
\label{fig:sen_des} }

\RawFloats
\capbtabbox{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Class name} & \textbf{precision} & \textbf{Recall} & \textbf{F1} & \textbf{Support}         \\ \hline
Defamation          & 0.30               & 0.72            & 0.42        & \cellcolor169 \\ \hline
Fake                & 0.67               & 0.84            & 0.77        & \cellcolor334 \\ \hline
Hate                & 0.44               & 0.80            & 0.57        & \cellcolor237 \\ \hline
Offensive           & 0.46               & 0.79            & 0.59        & \cellcolor219 \\ \hline
W.avg/Total         & 0.50               & 0.80            & 0.62        & 959                      \\ \hline
\end{tabular}}{%
\caption{Results for various model representations, evaluated on a subset of the MITRE and NIST dataset.}
\label{fig:ndcf_results}
}
\end{floatrow}
\end{figure}

% \begin{figure}[!h]
% \begin{floatrow}
% \RawFloats
% \capbtabbox{%
% \begin{tabular}{|l|l|}
% \hline
% \textbf{Name} & \textbf{Description}                                                        \\ \hline
% Bluetooth       & BLE  strength                                                            \\ \hline
% Accelerometer   & linear acceleration                                                      \\ \hline
% Gyroscope       & angular velocity                                                         \\ \hline
% Magnetometer    & \begin{tabular}[c]{@{}l@{}}magnetic \\ aberration\\ changes\end{tabular} \\ \hline
% Attitude        & roll, pitch, yaw                                                         \\ \hline
% Gravity         & \begin{tabular}[c]{@{}l@{}}Gravity along \\ X, Y, Z axes\end{tabular}    \\ \hline
% Altitude        & \begin{tabular}[c]{@{}l@{}}atmospheric\\ pressure changes\end{tabular}   \\ \hline
% Compass         & \begin{tabular}[c]{@{}l@{}}orientation \&\\  direction\end{tabular}      \\ \hline
% \end{tabular}}{
% \caption{Descriptions of mobile sensors present in both datasets.}
% \label{fig:sen_des} }

% \RawFloats
% \capbtabbox{%
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \textbf{Network} & \textbf{Train Set} & \textbf{nDCF} \\ \hline
% ConvGRU & MITRE & 1.02 \\ \hline
% RNN (GRU) & MITRE & 0.97 \\ \hline
% Feed Forward & MITRE & 0.77 \\ \hline
% \textbf{Conv1D} & \textbf{MITRE} & \textbf{0.58} \\ \hline
% Conv1D (MaxPool) & MITRE & 0.81 \\ \hline
% Conv1D (Dilation) & MITRE & 0.70 \\ \hline
% C-SVC & MITRE & 0.99 \\ \hline
% Nu-SVC & MITRE & 0.77 \\ \hline
% XGBoost & MITRE & 1.02 \\ \hline
% RF Classifier & MITRE & 1.04 \\ \hline
% RF Regressor & MITRE & 0.85 \\ \hline
% RF Histogram (Regressor) & MITRE & 0.90 \\ \hline
% Naive Bayes & MITRE & 0.92 \\ \hline
% GRU & NIST & 0.28 \\ \hline
% \textbf{ConvGRU} & \textbf{NIST} & \textbf{0.16} \\ \hline
% \end{tabular}}{%
% \caption{Results for various model representations, evaluated on a subset of the MITRE and NIST dataset.}
% \label{fig:ndcf_results}
% }
% \end{floatrow}
% \end{figure}
